Dynamic Pricing and Advertising with Demand Learning

We consider a novel pricing and advertising framework in which a seller not only sets the product price but also designs flexible advertising schemes to influence customers' valuations of the product. We impose no structural restriction on the seller's feasible advertising strategies and allow her to advertise the product by disclosing or concealing any information. Following the information design literature, we model this fully flexible advertising as the seller choosing an arbitrary information policy that signals the product quality to customers. Customers observe the advertising signal and form a Bayesian posterior belief over the product quality. We investigate two questions in this work: (1) What is the value of advertising? To what extent can advertising enhance a seller's revenue? (2) Without any a priori knowledge of the customers' demand function, how can a seller adaptively learn and optimize both pricing and advertising strategies using past purchase responses? To study the first question, we quantify the value of advertising by comparing the optimal revenue from jointly designing advertising and a single posted price with the optimal revenue from pricing alone. We show that advertising can increase revenue by at most a factor of two, and this bound is tight. For the second question, we study the seller's dynamic pricing and advertising problem under demand uncertainty. Our main result for this question is a computationally efficient online algorithm that achieves the optimal $O(T^{2/3} (m\log T)^{1/3})$ regret rate when the valuation function is linear in the product quality. Here, $m$ is the cardinality of the discrete product quality domain and $T$ is the time horizon.

==> Paper/apx-proof-rounding-general.tex <==

% In this subsection, 
% we provide the analysis for the rounding procedure 
% $\Round(\cdot, \cdot)$.
% We first provide the proof for 
% \Cref{lem:feasibility adver} which states that
% the output price and the output advertising strategy 
% from Procedure \ref{algo_construction_adver_general} indeed have 
% the desired property that we want. 
% Then we prove \Cref{lem:discretization error} which 
% states that the revenue loss
% is at most $2\varepsilon$ after Procedure \ref{algo_construction_adver_general}.


% \subsection{Proof of \texorpdfstring{\Cref{lem:no bad posterior}}{}}
% \label{proof of no bad posterior}
% \nobadposterior*


% \subsection{A rounding procedure to bound the discretization error}
% \label{subsec:rounding}
% \input{OR-23/4-1-rounding}




% \subsection{Details of Procedure \ref{algo_construction_adver_general}}
% \input{OR-23/procedure2}


% \subsection{Proofs of \texorpdfstring{\Cref{lem:feasibility adver} and \Cref{lem:revenue guarantee}}{}}
% \label{proof of feasibility adver}
% \label{proof of revenue guarantee}
% In this subsection, 
At a high-level the argument is as follows. Given an input price $\price$,
Procedure~\ref{algo_construction_adver_general} outputs the closest price $\newPrice\in\discPrice$
that satisfies $\price - 2\varepsilon \le \newPrice \le \price -\varepsilon$. 
Given an input advertising $\distOfMean$, 
for every posterior mean $\posteriorMean \in \supp(\distOfMean)$ and $\posteriorMean\notin \discPostMeanSpace_{\newPrice}$, 
with \Cref{lem:binary support},
there must exist two qualities $\qualityVal_i, \qualityVal_j$ where $i< j$ such that 
$\{i'\in[\stateNum]:\distOfMean_{i'}(\posteriorMean) > 0\} = \{i, j\}$.
For such posterior mean $\posteriorMean$, 
Procedure~\ref{algo_construction_adver_general} first identifies the 
critical type $x = \inverseVal(\price, \posteriorMean)$ and 
$x^\dagger = \inverseVal(\newPrice, \posteriorMean)$ where 
$x^\dagger$ lies within a grid $((z-1)\varepsilon, z\varepsilon)$ for some $z\in\N^+$.
Then, Procedure~\ref{algo_construction_adver_general} utilizes 
the critical-type function  $\inverseVal(\newPrice, \cdot)$ for the constructed price $\newPrice$
to find two posterior means
$\leftPosteriorMean, \rightPosteriorMean$ 
such that they satisfy:
$\inverseVal(\newPrice, \leftPosteriorMean) = z\varepsilon$ and
$\inverseVal(\newPrice, \rightPosteriorMean) = (z-1)\varepsilon$. 
\footnote{To see that such $\leftPosteriorMean$ and $\rightPosteriorMean$ always exist, note that because the valuation function 
is assumed to be monotone increasing in type $\theta$ (see Assumption \ref{assump:1a}), given any $\theta, 
p,q$, 
%critical type $\kappa(\price,q)$ is the unique solution to $v(\theta, q)=p$. That is for any $\theta,q,p$ 
if we have $v(\theta,q)=p$, then $\kappa(\price,q)=\theta$. Therefore, $\leftPosteriorMean$ and $\rightPosteriorMean$ are the values of $q$ satisfying $v(z\epsilon, q) =\newPrice$ and $v((z-1)\epsilon, q) =\newPrice$, respectively. Now, 
under linearity in quality, $v(\theta, q)$ is continuous in $q$ for any given $\theta$, which means that 
%for any $\theta, p$, there exists $q$ such that $v(\theta, q)=p$. Then, substituting $\theta=z\epsilon, (z-1)\epsilon$, and $\price=\newPrice$, we have that 
such solutions $\leftPosteriorMean$ and $\rightPosteriorMean$ always exist.}
To construct a feasible 
advertising strategy, we then round $\leftPosteriorMean$ up to be $\qualityVal_i$
when $\leftPosteriorMean < \qualityVal_i$ happens
and round $\rightPosteriorMean$ down to be $\qualityVal_j$ when 
$\rightPosteriorMean > \qualityVal_j$ happens.
By \Cref{assump:valuation}, and together with \Cref{lem:no bad posterior},
we can also show that the constructed
two posterior means $\leftPosteriorMean, \rightPosteriorMean$
satisfy
(a): $\leftPosteriorMean < \posteriorMean < \rightPosteriorMean$; 
and moreover (b): $\inverseVal(\newPrice,\leftPosteriorMean) \leq 
\inverseVal(\price, \posteriorMean)$, 
$\kappa(\newPrice,\rightPosteriorMean) \leq 
\kappa(\price, \posteriorMean)$.
The relation (a) enables us to decompose the probability over this posterior mean $\distOfMean(\posteriorMean)$
into probabilities over the two posterior means $\leftPosteriorMean, \rightPosteriorMean$ while still 
satisfying \eqref{bayes consistency} condition. 
Together with the monotonicity of demand function $\demand$,
the relation (b) can guarantee that the revenue of the output from Procedure \ref{algo_construction_adver_general} is $2\varepsilon$-approximate of the revenue of the input.



% \begin{lemma}
% \label{lem:discretization error no Lipschitz general}
% For any preference $F$, we have
% $\Rev(\optPrice, \optAdver) - 
% \Rev(\discretizedOptPrice, \discretizedOptAdver) 
% \le 
% 2\varepsilon $.
% \end{lemma}

% \subsection{Proof of \texorpdfstring{\Cref{lem:revenue guarantee}}{}}
% \label{proof of revenue guarantee}













